High Throughput Software for Powder Diffraction and its Application to Heterogeneous Catalysis

In this thesis we investigate high throughput computational methods for processing large quantities of data collected from synchrotrons and their application to spectral analysis of powder diffraction data. We also present the main product of this PhD programme, specifically a software called 'EasyDD' developed by the author. This software was created to meet the increasing demand on data processing and analysis capabilities as required by modern detectors which produce huge quantities of data. Modern detectors coupled with the high intensity X-ray sources available at synchrotrons have led to the situation where datasets can be collected in ever shorter time scales and in ever larger numbers. Such large volumes of datasets pose a data processing bottleneck which augments with current and future instrument development. EasyDD has achieved its objectives and made significant contributions to scientific research. It can also be used as a model for more mature attempts in the future. EasyDD is currently in use by a number of researchers in a number of academic and research institutions to process high-energy diffraction data. These include data collected by different techniques such as Energy Dispersive Diffraction, Angle Dispersive Diffraction and Computer Aided Tomography. EasyDD has already been used in a number of published studies, and is currently in use by the High Energy X-Ray Imaging Technology project. The software was also used by the author to process and analyse datasets collected from synchrotron radiation facilities. In this regard, the thesis presents novel scientific research involving the use of EasyDD to handle large diffraction datasets in the study of alumina-supported metal oxide catalyst bodies. These data were collected using Tomographic Energy Dispersive Diffraction Imaging and Computer Aided Tomography techniques.

==> Notes.tex <==

Dinnebier book: TWO-DIMENSIONAL DETECTORS The first two-dimensional detector in X-ray diffraction
was conventional film. It remained for decades the detector of choice for both single crystal as
well as powder diffraction experiments. In the field of two-dimensional detection it was surpassed
initially by image plates and later by CCD cameras (Figure 14.1). Today virtually no film is in
use, with perhaps the exception of Polaroid used for single-crystal images. To be able to compare
various detectors with one another, and to select the most appropriate detector for a specific
experiment, certain key technical qualities are important. These are in general the detective
quantum efficiency, the spatial response characteristics, the size, speed and dynamic range.

Dinnebier book: CCD Detectors Probably the most widely used detector type in X-ray crystallography
is the CCD camera. These detectors are in use in many fields and their general ongoing development
has been of benefit to the relatively small X-ray detector segment. The great advantages of these
detectors are their high resolution and short readout times. This is of importance especially in
single-crystal diffraction in which dead-times can make up a great part of the measurement time.
The drawbacks stem from three basic elements of the detector. First, the fluorescent screen has to
be optimised for the required wavelength: higher energy radiation requires a thicker layer to fully
absorb the incident rays. Thicker layers are disadvantageous as the PSF increases with the
thickness of the layer due to the spherical dissipation of excited electrons within the fluorescent
layer. Second, fibre optical tapers channel the light from the large fluorescent layer to the
smaller CCD chip. The tapering often leads to an imperfect representation of the original image
onto the CCD. This has to be corrected as much as possible within the detector electronics
(firmware). Some detectors have a CCD area of equal size to the fluorescent layer and can
circumvent this source of errors. Finally, one major drawback is the substantial dark current from
the CCD chip, which requires permanent cooling to reduce.

Dinnebier book: Imaging Plate Detectors Imaging plates were the first digital technology to replace
films in synchrotron and laboratory equipment. The concept is extremely simple. A layer of
BaF(Br,l):Eu21 which contains colour centres is deposited on a robust filmlike base ''plate''. The
plate is then exposed to X-rays. The image is later scanned by an online, or a more cumbersome
offline, scanner. Scanning the image consists of exciting the colour centres and then detecting the
induced radiation. Stimulating colour centres does not require much energy, generally red lasers
suffice. The stimulated green light is detected by a photomultiplier following the path of the
laser. The great advantages of imaging plates are their large size, low cost and their high dynamic
range. The latter quality has made it the detector of choice for two-dimensional powder
diffraction. Their major drawback is the high dead time associated with the time-consuming
scanning. This can take the best part of two minutes for large images. Rigaku MSC has developed a
practical solution to this problem. The detector system consists of two or even three detectors.
When one is being scanned the other can be exposed. A precision rotation system transports the
imaging plate from one position to the other. The future for this detector type does seem rather
bleak, though, especially in view of flat panel detectors and the single photon counting hybrid
pixel detectors.

Dinnebier book: Disadvantages of energy dispersive powder diffraction are the low resolution
obtained due to the limited energy resolution of the detectors, making it difficult to determine
accurate unit cell parameters. Fluorescence lines and absorption edges will also influence the
collected spectrum and it is generally difficult to obtain structural information, e.g. from
Rietveld refinement, from energy dispersive diffraction data. Angle dispersive diffraction is used
for most X-ray powder diffraction experiments using conventional or synchrotron sources. A
monochromatic X-ray beam is used, and the scattered intensity is recorded as a function of
diffraction angle. Very good unit cell parameters can be obtained and it is possible to collect
data that are suitable for structural investigations using Rietveld refinement. The time resolution
obtained depends strongly on the detector system. The detector may be a point detector, a
one-dimensional (position sensitive) detector or an area detector. The use of one- or
twodimensional detectors significantly increases the counting efficiency, as a large part of the
pattern is collected simultaneously. In addition, it is important for time-resolved (and
temperature resolved) powder diffraction experiments to collect the total powder diffraction
pattern in the shortest possible time, preferably simultaneously collecting the entire pattern.
This is not only to improve the time resolution; if a scanning detector (point detector or small
position sensitive detector) is used, the material may change between the start and the end of the
scan. Thus, analyses of the patterns, especially when extracting structural information, may be
problematic. When collecting the entire pattern using a large position sensitive or area detector,
any changes taking place during measurement/exposure is reflected in the entire collected pattern.

Dinnebier book: The use of two-dimensional detectors, where the entire, or a significant part of,
the Debye-Scherrer rings are collected will, in addition to improved counting statistics, limit the
negative effect of small samples, i.e. non-statistical number of crystallites and, to some extent,
texture. Geometric effects of these detectors are described in detail in Chapter 14. The use of
high-resolution synchrotron X-ray powder diffraction for time-resolved in situ studies is limited
by the obtained intensity, and thereby the time resolution. The use of multiple analyser crystals
will reduce the time required for each data set. In addition, the availability of high-resolution
powder diffractometers on insertion device beam lines (wiggler or undulator) with multiple analyser
crystals, such as ID31 at ESRF or 11-ID at APS, makes it possible to perform experiments where very
high-resolution data are obtained with good time resolution. This development will significantly
contribute to the use of in situ powder diffraction for attacking increasingly more complex
problems.
















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

key words: alumina(), gamma alumina(), molybdenum, molybdenum (tri)oxide, heterogeneous,
production, metal oxide, support (catalytic support), impregnate, raman, nickel(), cobalt

Plan:

1. Introduction
 - Heterogeneous catalysis
 - Importance of industrial catalysis with examples.
 - Industrial production of catalysis including extrudates. (Importance of catalytic supports)
 - Study of extrudates to date including Raman.
 - Statement concerning work.

2. 2D static studies of Mo and Co on alumina
 Review and Ang. Chem. (preparation study)
 + SDMJ unpublished work.

3. 2D static + 1D space/time study of Ni on alumina. (preparation study)

4. 2D space/time study of Mo on alumina.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


make essay1 in a single chapter

unify biblios and nomenclatures

add back projection algorithm symbols to nomenclature

update Trolltech name and web link












%XXXXXXXXXXXXXXXXXXXXXXX

in the end:

check all abbreviations are in use

all biblio are referenced





%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
Simon notes:

Title: Development of software for batch processing and visualisation of powder diffraction data.

In section 2 (intro) make a note about the name of the software. it is not only about EDD as will
be seen in section 12.

the curve-fitting model can be used for general spectral analysis

11 examples of use of EasyDD: the study of alumina supported metal oxide catalyts

11.1 Introduction: Show case studies where EasyDD has been used in the study of alumina supported
metal oxide \catalyst s [all these from Beale  paper]

 Extrudates as preferred industrial support for hetergeneous \catalyst s
What is the prep procedure
 Preparation procedure key to their perfomance.

 Systems under study : application of the catalyst systems

11.2 Sample description and preparation

11.3 Results

11.3.1: 2D Spatial studies using energy-dispersive diffraction Review of Beale JBBW 2007 Molybdenum
and Cobalt on alumina

TEDDI description - direct imaging - EasyDD gives you direct images (after beam & count rate
correction)

11.3.2: 2D Spatial/temporal studies using energy-dispersive diffraction Work in progress. Letti et
al. Unpublished.  Nickel on alumina

Again using TEDDI but this time spatial/temporal mode - again images are direct or need
deconvoltuion (Not yet implented in EasyDD)

11.3.3: 3D Spatial/temporal studies using angle-dispersive diffraction Work in progress. Jacques et
al. Unpublished  Molybdenum on alumina

Using CAT like ADD (demonstrated by Bluet et al). several processing stages: data from 2d to 1d
(DATASQUEEZE), images are not direct but sinograms require reconstruction --> before doing this we
need corrections for motor positions(arising because of the nature of data acquision).

 11.4 Conclusions
Science conclusions Development conclusions: shortfalls of esyEDD

12 Future developments



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Include literature review file in the thesis





see "Comparison of Pawley \& LeBail methods" and "Direct Methods" in BBK course

Book Messerschmidt 2007: The term "direct methods" denotes those methods which try to derive the
structure factor phases directly from the observed amplitudes through mathematical relationships.

Book Messerschmidt 2007 (175): "Improving the agreement" between the observed and calculated data
can be done by different criteria to measure the agreement. The most commonly used measure is the
L2 norm of the residuals, which is simply the sum of the squares of the differences between
observed and calculated data, [equation] where wi is the weight of observation, yi and Mix is the
calculated value of observation i given the parameters x. The least-squares refinement now searches
for the set of model parameters that give the minimum variance of the observations. One problem of
the L2 norm is that it is very sensitive against large deviations, which occur especially during
the early stages of refinement. To overcome this, it may be better to refine against the L1 norm:
L1x i wi yi Mix 72 which is the sum of the absolute value of the residuals. However, to date this
technique has not been used in macromolecular crystallography.

Book Messerschmidt 2007: In Prince and Boggs (1999), two useful ways of solving the minimisation
problem are described, the Gauss-Newton algorithm and the Quasi-Newton method.

Book Messerschmidt 2007: All of the above-mentioned refinement procedures are based on the
leastsquares method. The radius of convergence for this method is not very high because it follows
a downhill path to its minimum. If the model is too far away from the correct solution, the
minimisation may end in a local minimum corresponding to an incorrect structure. Brünger and
colleagues (Brünger et al., 1987, 1993) introduced the method of simulated annealing (SA), which is
able to overcome barriers in the L2-function and find the correct global minimum. The SA algorithm
requires a mechanism to create a Boltzmann distribution at a given temperature T and an annealing
schedule T1  T2   Tl at which the Boltzmann distribution is computed. There exist several methods
to be

Book Pecharsky Z 2005: The shapes of real Bragg peaks, which are the results of convoluting
multiple instrumental and specimen functions (Eq. 2.45), are rarely described well by simple
Gaussian or Lorentzian distributions, especially in x-ray diffraction. Usually real peak shapes are
located somewhere between the Gauss and Lorentz distributions and they can be better represented as
the mixture of the two functions.' An ideal way would be to convolute the Gauss and Lorentz
functions in different proportions. This convolution, however, is a complex procedure, which
requires numerical integration every time one or several peak shape function parameters change.
Therefore, a much simpler linear combination of Gauss and Lorentz functions is used instead of a
convolution, and it is usually known as the pseudo-Voigt function (Eq. 2.5 1). The Gaussian and
Lorentzian are mixed in q to 1-q ratio, so that the value of the mixing parameter, q, varies from 0
(pure Lorentz) to 1 (pure Gauss). Obviously, q has no physical sense outside this range.

Book Pecharsky Z 2005: Maximum entropy method is a powerful numerical technique, which is based on
Bayesian estimation theory and is often applied to derive the most probable values of missing data.
For example, rolling a dice with six faces numbered 1 through 6 gives equal probability to see each
face up, pi = 116, assuming a completely random distribution. In this case, the average value of
multiple observations is (1+2+3+4+5+6)/6 = 3.5. The problem is in finding the probability of events
(faces up) when the distribution is not random and only the average is known, e.g. when the average
is 2.5. The maximum entropy method results in the highest unbiased unique probability of events
(e.g. faces up in the case of a dice) using the entropy function, Cpiloppi. This method, similar to
the genetic algorithm approach, finds applications in various fields of scientific analysis,
especially in image processing and reconstruction.' In powder diffraction, the maximum entropy
technique can be and is successfully employed both to restore the lost phase angles2 and to
determine the relative intensities of the overlapped reflection. Crystal structure determination
using the maximum entropy approach results in solving the phase problem and therefore, it is a
reciprocal space method.


Book Pecharsky Z 2005: Even if the refinement is stable, it should be terminated at a certain
point. Because of the finite accuracy of both the data and computations, it is unrealistic to wait
until increments of all \ls\ parameters become zero. The latter usually never happens anyway due to
simplifications introduced in the non-linear least squares algorithm (see Eq. 6.9 in section 6.6).
In addition to the stabilization of all figures of merit near their respective minima, another
important factor that should be considered is the relationships between the increments and
corresponding standard deviations after each \ls\ cycle. It is commonly accepted that when all
residuals converge and stabilize at their minima, and when the absolute values of all increments
become smaller than the estimated standard deviations of the corresponding free variables,' the
least squares refinement may be considered converged (indeed, the model must remain rational).

see section 10 of numerical recipes on function minimisation algorithms

page 820-> of numerical recipes on baysian theory and maximum entropy

see "Clark 1995" for profile fitting without knowledge of structural or unit cell parameters

Dong S 1999: The base algorithm was conceived to work as an unconstrained profile fitting (Pattern
decomposition) or a constrained modelling of the whole powder pattern (Pawley method), by which
peak positions or lattice parameters, respectively, can be re®ned by least squares.

Getting Started with Rietveld: A beam impinging on the sample will find a representative number of
crystallites in the right orientation for diffraction

Getting Started with Rietveld: Powder diffraction offers fewer observations and worse
peak-to-background than single crystal diffraction

Joubert 2002: A pattern is first calculated from the known structure information: the nature of the
phases in the sample, atomic positions and the nature of the atoms at each site according to the
structure prototype, approximate line profiles and lattice parameters. The calculated pattern is
compared with the experimental (observed) one and the parameters defining the calculated pattern
are iteratively refined by a non-linear least-square method in order to obtain the best agreement
between the two patterns, by minimising the function: where y stands for the observed (ohs) and
calculated (talc) intensities, the summation being done over each point of the diffraction pattern.
The parameters, which can be refined and therefore experimentally determined include background
parameters, line profile parameters (derived from the observed line shapes), lattice parameters
(derived from the observed line positions), atomic positions, displacement factors and occupancy
factors (derived from the line intensities). This paper will be devoted to what can be obtained
from this latter parameter in the frame of the thermodynamic modelling of a particular phase.

LangfordL1996: The indexing of powder diffraction patterns, i.e. the determination of crystal
symmetry, unit cell dimensions and hkl indices of each reflection, is an essential step in ab
initio structure determination.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\Hs}      {\hspace{-0.6cm}} %
%\newcommand{\CIF}     {\centering \includegraphics[width=1in, trim = 10 0 130 40]} %
%\newcommand{\Mini}    {\begin{minipage}[b]{0.27\textwidth}} %
%\newcommand{\Vmin}    {\vspace{0.5cm}} %
%
%\begin{figure}
%%
%\centering %
%\subfigure[ambient]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/ambient}
%\end{minipage}}
%\Hs %
%\subfigure[ramp1]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/ramp1}
%\end{minipage}}
%\Hs %
%\subfigure[ramp2]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/ramp2}
%\end{minipage}}
%\Hs %
%\subfigure[ramp3]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/ramp3}
%\end{minipage}} \Vmin
%
%%%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
%
%\centering %
%\subfigure[ramp4]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/ramp4}
%\end{minipage}}
%\Hs %
%\subfigure[ramp5]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/ramp5}
%\end{minipage}}
%\Hs %
%\subfigure[ramp6]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/ramp6}
%\end{minipage}}
%\Hs %
%\subfigure[ramp7]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/ramp7}
%\end{minipage}} \Vmin
%
%%%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
%
%\centering %
%\subfigure[ramp8]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/ramp8}
%\end{minipage}}
%\Hs %
%\subfigure[ramp9]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/ramp9}
%\end{minipage}}
%\Hs %
%\subfigure[ramp10]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/ramp10}
%\end{minipage}}
%\Hs %
%\subfigure[ramp11]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/ramp11}
%\end{minipage}} \Vmin
%
%%%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
%
%\centering %
%\subfigure[ramp12]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/ramp12}
%\end{minipage}}
%\Hs %
%\subfigure[ramp13]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/ramp13}
%\end{minipage}}
%\Hs %
%\subfigure[final0]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/fin0}
%\end{minipage}}
%\Hs %
%\subfigure[final1]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/fin1}
%\end{minipage}} \Vmin
%
%%%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
%
%\centering %
%\subfigure[final2]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/fin2}
%\end{minipage}}
%\Hs %
%\subfigure[final3]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/fin3}
%\end{minipage}}
%\Hs %
%\subfigure[final4]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/fin4}
%\end{minipage}}
%\Hs %
%\subfigure[final5]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/fin5}
%\end{minipage}} \Vmin
%
%%%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
%
%\centering %
%\subfigure[final6]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/fin6}
%\end{minipage}}
%\Hs %
%\subfigure[final7]%
%{%\label{fig:mini:subfig:a}
%\Mini \CIF {g/fin7}
%\end{minipage}}
%
%\caption{Sums of the diffraction patterns of the reconstructed images for the individual data sets.
%The range of the $x$-axis in all sub-figures is 0-10. The range of the $y$-axis for sub-figures k,
%l, o, p, q, r, s, u and v is 0-300000, while for the rest it is 0-350000. \label{sumOfPatterns}}
%\end{figure}








XXXXXXXXXXXXXXXXXXXXXXXXXXXXXX Store

The parameters in the \Rietveld\ refinement may be divided into three main categories which
represent different aspects of the profile. These categories are: structural, background, and
profile parameters. The structural parameters determine the positions and integrated intensities of
the \Bragg\ reflections. Atomic positions in the unit cell, displacement parameters and site
occupancies determine integrated intensities while unit cell parameters determine peak positions.
The quality of pattern generally imposes a limit on the maximum number of structural parameters
that can be safely refined. The background parameters describe the background contribution which
superimposes on the diffraction signal. This contribution may include diffuse elastic and inelastic
scattering from the sample and environment, electronic noise, air scattering, and many other
unwanted signals. As Bragg signal is highly structured, it is usually easy to separate from the
background. The role of the profile parameters is to describe the shape of peaks. Line broadening
mainly arises from the instrument resolution, with possible contribution from the sample itself due
to crystalline size and micro strain. Further refinement parameters may be added for special
purposes to these categories \cite{AlbinatiW1982, BookCopley2001}.

In the \Rietveld\ approach the calculated intensity at coordinate $x_{i}$ is given by

\begin{equation}\label{RietveldEq}
    \CCR(x_{i}) = \sum_{j} \II_{j} \POF_{j} \RPF(x_{i} - x_{j}) \ +
    \  \BCR(x_{i})
\end{equation}
%
where the summation runs over all reflections contributing to the intensity at $x_{i}$. In this
relation, $\RPF$ is the reflection profile function, $\POF_{j}$ is a \preori\ function, and
$\II_{j}$ is the integrated intensity of reflection $j$ given by

\begin{equation}\label{IIEq}
    \II_{j} = \SFb \RM_{j} \LPF_{j} \left[ \sum_{i} \FO_{i} \SPF_{i} \, e^{2 \pi \IU (hx_{i} + ky_{i} + lz_{i}) - \TF_{i}} \right]^{2}
\end{equation}
%
where $\SFb$ is the scale factor that transforms intensities from arbitrary to physical units,
$\RM_{j}$ is the reflection multiplicity, $\LPF_{j}$ is the \Lorentz\ polarisation factor, $x_{i}$,
$y_{i}$, $z_{i}$ are the fractional coordinates of atom $i$, $hkl$ are the \Miller, $\FO_{i}$ is
the fractional occupancy for the $i^{th}$ atomic site, $\SPF_{i}$ is the scattering power factor
(i.e. scattering factor for X-rays and nuclear scattering length for neutrons) and $\TF_{i}$ is the
temperature factor \cite{LangfordL1996}.

xxx

[F]The distinctive feature of the Pawley \whpade\ procedure is that the refinable parameters
include the integrated intensities of the individual peaks, alongside the other refinable variables
such as profile and background parameters. It relies on the assumption that the diffraction peaks
have independent variable intensities. The method was first proposed by \Pawley\ \cite{Pawley1980,
Pawley1981} to refine unit cell parameters and obtain integrated intensities. In this method, the
profiles are modelled analytically with the widths being constrained by a \Caglioti\ law
\cite{CagliotiPR1958}

\begin{equation}\label{CagliotiEq}
    \FWaHM^{2} = U \tan^{2} \SA + V \tan \SA + W
\end{equation}
%
where $\CP$ are the \Caglioti\ parameters. The Pawley refinement generates a list of refined
parameters and indexed intensities that can be used as an input to other methods (e.g. direct
methods) to find structural information if required. Various statistical indicators and
figures-of-merit can be used to monitor the convergence and assess the results, as in the case of
\Rietveld. In this procedure, slack non-structural constraints are employed to overcome \ls\
ill-conditioning due to peak overlap \cite{Pawley1980, Pawley1981, Young1993}.

[F]Because the intensities are treated as refinable parameters, the \Pawley\ approach requires
handling matrices of considerable size. The procedure is therefore computationally expensive and
may impose a limit on the size of the problem to be solved. However, it provides full information
about covariance matrix and this can be a big advantage in some cases. The \Pawley\ procedure works
best when the diffraction pattern is relatively simple. When the number of independent diffraction
peaks is large, the \Pawley\ algorithm can become unstable, especially if there is severe overlap.
When the pattern is too complex, the algorithm usually suffers from ill-conditioning and negative
integrated intensities. The use of artificial constraints in the form of additional observations to
avoid negative intensities can bias the results. Other procedures, such as \Lebail, may be used to
avoid these problems which are inherent to the \Pawley\ procedure \cite{JansenPS1992a, David2004}.

[F]Like \Pawley, the \Lebail\ procedure is a pattern decomposition method. It is generally praised
for simplicity, robustness and speed, and hence it is the more popular and widely available of the
two. It is proposed by \Lebail, Duroy and Fourquet \cite{LeBailDF1988} as a simplification to the
\Rietveld\ procedure which requires atomic structure information that may not be available. In the
Le Bail method the \spagro\ and lattice parameters are employed as constraints with no explicit
reference to a crystallographic structural model. The method normally employs a nonlinear \ls\
routine to optimise the fit between the observed and the calculated patterns. In Le Bail, only
background, profile and lattice parameters are refined in the \ls\ cycles and hence the number of
refined parameters is not related to the number of diffraction peaks. Since the refined parameters
are very few (typically 10-20), the method is fast, efficient and stable. The \Lebail\ procedure
produces one set of peak intensities which fit the entire diffraction pattern. The \Rietveld\ and
\Lebail\ mainly differ in the calculated intensities as the Rietveld computes these intensities
from the structural model while the Le Bail obtains them from the preceding \ls\ cycle. At the
start of the Le Bail procedure, all calculated intensities are given an arbitrary value, usually
unity \cite{BookPecharskyZ2005}.

[F]The \Lebail\ algorithm is more popular than \Pawley\ and has been implemented in a number of
powder diffraction programs including several freely available softwares such as \GSAS\
\cite{LarsonV2004}. Furthermore, \Lebail\ is recognised as being fast, robust and more stable than
\Pawley. Intensities are refined in the \Pawley\ procedure but not in the \Lebail\ in which only
cell and profile parameters are refined while the intensities stay unchanged during the individual
\ls\ cycles. Consequently, in the \Pawley\ method a number of refined parameters equal to the
number of peaks should be included in the refinement. This factor may explain why \Lebail\ is
superior in terms of stability and speed. \Lebail\ also converges in some complex cases in which
\Pawley\ usually fails. However, \Lebail\ normally takes more \ls\ iterations to converge.
Moreover, higher precision is required in \Lebail\ for the unit cell parameters. Another advantage
of \Pawley\ is that it produces the covariance matrix which describes the correlation between the
intensities. This matrix can be used for further structure analysis \cite{Louer1998}.

The profile residual $\PR$ is described as a true quantity as it is based on the difference between
the experimental and calculated intensities. Of these figures-of-merit, the weighted profile
residual $\WPR$ and the goodness-of-fit index $\GoFI$ are the most meaningful statistical
indicators of the overall fit since the numerator is the quantity that is minimised in the \ls. The
goodness-of-fit index, which is widely used in the literature of powder diffraction, is considered
as one of the most important and reliable figures-of-merit. The expected residual $\ER$ is used in
the \Rietveld\ refinement to quantify the quality of the experimental data. The \strfac\ residual
$\SFR$, which gives an indication of the reliability of the structure, is biased towards the chosen
structural model and is not widely used in powder refinement. The \Bragg\ residual $\BR$ is based
on the intensities deduced from the model and hence is biased in favour of the used model. It is
highly dependent on the procedure in which the observed integrated intensities are estimated, and
may be described as an artificial quantity created to emulate single crystal residual. However,
$\BR$ is an important statistical indicator in whole pattern structure modelling though has no
value in whole pattern decomposition because only observed \Bragg\ intensities are meaningful in
pattern decomposition. The profile residuals depend on the absolute number of counts $\OCR_{i}$
which is reasonable for pure \Bragg\ scattering with no background. In the presence of background
scattering, which is unavoidable in practical situations, the counting statistics will be improved
resulting in a better profile fit for higher background contamination. Consequently, these
residuals can lose their meaning unless the background is subtracted \cite{JansenSW1994,
MccuskerDCLS1999}.

Discrepancies in the figures-of-merit (FoM) values have been reported in the literature of powder
refinement not only between different methods when applied to the same data, but also between
different implementations of the same method. The refinement programs can refine many variables at
the same time which may cause strong parameters correlation leading to wrong results and misleading
statistical indicators. In such cases, the figures-of-merit must be examined and assessed carefully
to avoid being a source of erroneous confidence. As the universality and objectivity of some of
these FoM may be questioned, the definition of these figures for each method must be known for fair
comparison with other methods. Moreover, the user should try to avoid using single or controversial
FoM and rely instead on a collection of obvious and generally accepted indicators.

Several highly-structured databases, such as Powder Diffraction File, have been created to store
these data for such uses.

\Pd\ is a powerful tool for the identification of phases present in a powder sample.

This is an important and widely used application of \pd\ technique in analysing multiphase samples.

The model introduces a great simplification to the mathematics of \diffraction\ calculations, and
when combined with the abstract concept of reciprocal lattice it simplifies the experimental
measurement of \difpat s.

However, in the case of single \crystal\ \diffraction\ this information is distributed in a 3D
space, whereas in the case of \pd\ the 3D information is compressed into one dimension. This
usually results in a considerable overlap of peaks in \pd\ patterns, especially at higher \scaang,
leading to severe technical difficulties in extracting the 3D structure from the 1D \difpat.

In the last 60 years, synchrotron facilities around the world constantly evolved to meet the ever
increasing demands of science and technology.

The properties of SR for \Xray\ crystallography have been recognised and harnessed as \synch s with
the requisite machine energies became available. \Synch\ radiation sources provide intense beams of
X-rays for cutting-edge research in a broad range of scientific disciplines.

Though the divergence of the pencil beam is small, the cross sectional area at the location of
experiment is in some cases can be several mm$^2$. However, in many cases the emerging beams are
extremely fine just a few microns across.

Due to its unique properties such as high intensity, collimation, tunable energy and high degree of
polarisation, \synrad\ has been exploited in many scientific and technological applications in
various fields. These include physics, chemistry, crystallography, medicine, materials science,
forensic science, and archaeology. In recent years synchrotron facilities have become widely used
as preferred radiation sources for performing \Xray\ \diffraction\ measurements. These powerful
sources, which are thousands to millions of times more intense than laboratory \Xray\ sources, have
become indispensable tools for a wide range of crystallographic structural investigations. The
scientific developments of Synchrotrons and crystallography are closely linked as crystallographic
research is one of the main users of \synrad. As \synch s provide high intensity light across a
wide range of electromagnetic spectrum, SR is used as a powerful probe to examine the underlying
structures and properties of matters, and to analyse various physical, chemical and biological
processes. Synchrotron research is developing rapidly in a number of key areas, with a strong
evidence of increasing demand for SR world-wide for both scientific and industrial applications.
This may be reflected by the increase of the number of \synch s built in the last decades and the
strong competition on beam time. Some industrial and strategic applications of \synrad\ have a
confidential nature, and hence it is difficult to make a comprehensive list of SR applications.

For example, powder diffraction data can be used in conjunction with a \twstme\ procedure for
\abinitio\ structure determination by conventional methods such as direct methods

$\OCR$ and $\CCR$ are the observed and calculated count rate respectively, $\SW$ is the statistical
weight, $\NoO$, $\NoP$ and $\NoC$ are the numbers of observations, adjusted parameters in the
calculated model, and applied constraints respectively, $\OII$ and $\CII$ are the observed and
calculated integrated intensity respectively, and $i$ and $k$ are counting indices.

It should be remarked that the \ls\ iteration cycles should be terminated when a certain realistic
error tolerance is reached without waiting the parameters increment to converge to zero. This is
due to the limits on the accuracy of both the data and the calculations, and therefore excessive
iteration will be waste of computational resources. Furthermore, absolute convergence never happens
in most cases.

Other statistical energy optimisation methods have also been employed in \pd\ pattern refinement.
One of the problems in these methods is the presence of multiple local minima on the way to the
global minimum, thus making the search for the lowest energy very slow. Different techniques have
been developed to speed up the process. For example, simulated annealing, which resembles the
physical process of annealing by virtually heating a sample to a certain temperature followed by
slow cooling over time, has been employed to explore local minima quickly by generating multiple
trial models using Monte Carlo and grid search methods.

Some programs follow an intermediate approach between full- and reduced-pattern matching by taking
a full-profile unknown pattern and compare it to a database of reduced patterns.

In our investigation (see \S\ \ref{Ex3}) we used \Datasqueeze\ in batch mode to convert in a single
run a large number of \CCDs\ image files (over 21000) obtained from \ESRFs\ to $x$-$y$ data files.

The program is also capable of doing model fitting on a variety of input data and perform
calibration and correction of detector distortion, among other sorts of data processing and
analysis. Several commonly-used standard basis functions such as \Gauss ian, Lorentz ian,
polynomial, exponential and trigonometric are available for peak and background modelling.

such as programming language, platform (Windows, UNIX, etc.), sophistication, underlying
computational algorithms, reliability, user interface (GUI or command line), user-friendliness,
licensing (free or commercial), distribution (with or without source code), and so on

There is a graphical user interface and shell to \GSAS, called EXPGUI (by Toby), that can be used
to call the various \GSAS\ programs. EXPGUI, which is a separate add-on, provides access to a
limited range of the \GSAS\ capabilities. \GSAS\ includes a facility for interactive graphics
display based on the PGPLOT graphical subroutine library. Full range of \GSAS\ capabilities are
available only through the command-line type EXPEDT.

It can also be used for data manipulation and display, removing baselines, positioning of peaks,
changing peak parameters, and automation of common tasks with scripts. The program has a number of
features that make it flexible and user friendly. These include intuitive graphical interface,
support for user-defined fitting functions, graphic labelling and display of curves, and handy
methods for creating, positioning, removing and modifying basis functions.

The final decision should be based on good understanding and sound analysis

Data visualisation can be regarded as a high throughput process at least in some situations where
massive volumes of data are involved.

However, the user must take care of the data by placing the right files with the certain extension
in the right directory to avoid complications. Therefore, on invoking a particular function the
program will find only the relevant files when looking to the data source directory.

It is meant to be a tool for processing large quantities of data in a variety of formats with ease
and comfort using limited time and computing resources.

This is demonstrated by the growing use of automated and computerised data collection techniques on
one hand, and the availability of vast electronic storage with massive processing computational
power on the other.

The first is that of \DiamonD\ Light Source MCA files. These files have headers and footers to be
ignored. The rest of the file contains the intensity (number of counts) as a function of channel
number, where the channel number is implicit and hence is identified by the entry position. The
second format is that of ESRF MCA files. These files have only headers to be ignored, and the first
data line starts with `@A' with each 16 data entries being on a single text line ending with
backslash `$\backslash$'. Again, the data in these files are intensity versus implicit channel
number.

Therefore, the data in each file should be sectioned in rows corresponding to the detector rows.

This parameter is needed for tilt correction.

Text formatting can help to identify the distribution of the data and can be used to replace colour
coding as a generic and quick form of interpreting the data. However, formatting may incur a cost
in terms of output files size and processing time.

The data in any tab can also be exported as $xy$ text format for the use in other applications and
further processing or for archiving especially following corrections and modifications.
Intensities, refined parameters and statistical residuals can also be exported separately to
generic text files for further processing or for visualisation by other applications. The written
data are structured in a 2D matrix with the same dimensions as the tab. The spectrum of each voxel,
as represented by a cell in a tab, can be plotted using a 2D plotter which is described in \S\
\ref{2DPlotter}. The sum of all patterns in a tab can also be written to a text file and plotted on
the 2D plotter to compare with the individual patterns and to characterise the overall behaviour.
Rows, columns and cells in each tab can be managed and manipulated by 12 functions which include
delete, copy, exchange, rotate clockwise and anticlockwise and so on. Moreover, the tab can be
transposed by reflection across the $y=-x$ line.

On double-clicking a cell in a tab in the tab widget the plotter will be launched, if it was not
launched already, and the pattern of the selected cell is plotted.

All plotters are closed when the tab widget is cleared by removing all tabs.

It should be remarked that a form can be prepared in a simple text file, then copied and pasted
into existing form of the same dimensions. This simplifies the task of updating the forms when the
format of the form changes between two versions of the program.

The form therefore has two modes of launch, one from the plotter and the other from the main
window. In the first mode the form interacts with the plotter, i.e. the form automatically lists
the existing basis functions in the plotter. Moreover, the plotter is updated on modifying the
parameters of the basis functions in the form. In the second mode the form serves as a fitting
model for batch and multi-batch \curfit.

If the form is a child of the plotter, the plotter is dynamically updated on changing the fitting
function parameters such as position or FWHM. The form also has an $x$ range, that is the minimum
and maximum $x$ of the plotter frame when the form is created. The range is therefore controlled by
zooming the plotted pattern in and out. This range is used in the curve-fitting operations.

On performing batch fitting, a list widget for each refined tab is created where the statistical
indicators and refinement parameters, as well as intensity, are displayed. From this widget the
colour coding of the tab can be changed according to each one of these quantities.

The algorithm takes the image, which is a matrix of intensities, rotate it, and sum up these
values. The image may require padding with zeros to a power of 2 when applying a Fourier Transform.

Although these are lengthy calculations, they are carried out only once at the beginning of EDF
numeric conversion and the results are stored in a correction vector to be used in the following
multi-batch process. Hence, no significant extra time is spent on the tilt correction. In fact this
can result in a significant time save as the radial distance is calculated only once. However, the
assumption is that the tilt is the same for all the data processed in a single run of multi-batch
process.

Their use reduces the production cost and results in a better selectivity and hence less waste. []
\Catalyst s play a key role in industrial chemical transformations. By offering an
energetically-favourable reaction routes, they facilitate chemical processes under practical
physical conditions. [] and this fact indicates the importance of these agents in the chemical
industry [] Chemical industry therefore heavily relies on the use of \catalyst s in their
production processes.

Generally, the active sites in \hetcat s are on their surface. [] \Hetcat s paly a vital role in
chemical processes both in the lab and in the industry.

\begin{figure} [!h]
\centering
\includegraphics
[scale=0.35] {g/Ex1}
%
\caption[Detector signal from a Mo/Al$_2$O$_3$ \catalyst\ body]{Detector signal from a
Mo/Al$_2$O$_3$ \catalyst\ body (a) after drying at 120$^\circ$C and (b) after calcination at
500$^\circ$C (after Beale \etal\ \cite{BealeJBBW2007}).} \label{Ex1}
\end{figure}
%
Spectral patterns and tomographic images for the distribution of Mo/Al$_2$O$_3$ \catalyst\ (a)
after drying at 120$^\circ$C and (b) after calcination at 500$^\circ$C (after Beale \etal\
\cite{BealeJBBW2007}).
%
Some of the results of this investigation is presented in Figure \ref{Ex1}.

The results show both the precursor and the active \catalyst\ have an egg-shell distribution, where
the latter is independently confirmed by spatial Raman spectroscopy. Moreover, there was little
apparent migration of Mo during calcination.

The images were reconstructed by direct mapping without deconvolution.

\ProgName\ was the main tool used for visualisation, \curfit\ and analysis of this data collection.

This may confirm some of the experimental results and conclusions.


\begin{figure} [!h]
\centering
\includegraphics
[scale=0.6] {g/NiChlFirstStack}
%
\caption{Stack plot of the sum of total intensity of the nickel chloride data sets (first squeeze,
Sinograms).} \label{NiChlFirstStack}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure} [!h]
\centering
\includegraphics
[scale=0.6] {g/NiChlSecondStack}
%
\caption{Stack plot of the sum of total intensity of the nickel chloride data sets (second squeeze,
Sinograms).} \label{NiChlSecondStack}
\end{figure}


\item This PDP is observed from \sad\ = 1.07581, 1.07685, 1.36219, 2.62135, 2.63428. This apparently
comes from the precursor or some sort of impurity.

\item This PDP which apparently comes from the precursor is observed from \sad\ = 0.771562, 0.771782,
1.55882, 1.56048, 1.56554.

\item This PDP apparently comes from a transitional phase and is observed from \sad\ = 2.26629, 2.26726,
2.45957, 2.46046, 3.0197, 3.02373.

\item This is observed only from \sad\ = 1.13434. As it seems to be a combination of the two previous PDPs,
it is most likely that it comes from two overlapping peaks belonging to two previous phases.

\item This is observed from \sad\ = 1.88303, 1.99381, 1.99475, 2.36196, 2.76512, and it comes from \moltri.

\item This is observed from \sad\ = 2.08861, 2.08993, 2.10395, 2.10503, 2.11898, 2.11912, 3.40215,
3.41346, 4.36978, 4.36984, 4.84782, 4.84989, 5.03671, 5.03776, 5.53411. This PDP apparently comes
from \moltri.

[F]It should be remarked that the most prominent alumina peak consists mainly of two overlapped
\Bragg\ reflections which are the $hkl=224$ reflection (with relative intensity = 1 and
multiplicity = 8) and the $hkl=400$ reflection (with relative intensity = 0.516 and multiplicity =
4). The second largest alumina peak also consists of two main \Bragg\ reflections which are the
$hkl=220$ reflection (with relative intensity = 0.998 and multiplicity = 4) and the $hkl=004$
reflection (with relative intensity = 0.473 and multiplicity = 2). The combined intensity of these
peaks, as seen in Figure \ref{Ex3Image1}, reflects this weighted combined intensity. Also, the
alumina tomographic images, as seen in Figures \ref{5p76706-Par3} and \ref{4p08027-Par3}, represent
the combined effect of these overlapped peaks.

It should be remarked that the values of these angles are approximate and should be regarded as
labels, as they represent an average value of the large number of positions of the individual peaks
represented by that scattering angle.

[F]In the following we present some general conclusions that can be obtained from the analysis of
molybdenum data:
\begin{itemize}
\item It is evident that there is an alignment problem in some data sets, as discussed earlier. Also, the
sample is not evenly heated as one side can be seen cooler than the other due to the location of
the heating element (hot air blower). These problems should be addressed in the forthcoming
experiments.
\item As can be seen in Figures \ref{Ex32p10395-Par3} and \ref{AluminaPositionChange}, the situation is
hardly changing in the \stesta\ data sets, which is a sign of consistency.
\item The formation of various phases can be tracked during the ramp stages, as can be seen for example
in Figures \ref{MolStack}, \ref{sum3DPlot} and \ref{Ex32p10395-Par3}.
\item There is no simple analysis as the systems are very complex and it is not evident that each phase
distribution pattern belongs to a single phase.
\end{itemize}

%SSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSS
\section[3D Spatial/Temporal CAT Type ADD Studies (Ni)]{3D Spatial/Temporal CAT Type ADD Studies
of Preparation and Operation of Nickel Catalysts Supported on Alumina Extrudate} \label{Ex4}

This project involves analysis of data gleaned from the Nickel system*(s) studied in June 2009. In
the experiment a system was studied in-situ from preparation through to operation:

\begin{enumerate}

\item Pre calcined 3D measurement of air dried extrudate body — a collection of 2D slices at
different heights in the extrudate yielding a 3D map [11 slices \@ 1394 files per slice = 15,334
files each \@ 9.66 MB equates to 144 GB]

\item 2D + temporal measurement of the extrudate — similar to that carried out on the Mo sample
described in section 4.2.3

\item Post calcined 3D study of extrudate

\item 2D + temporal measurement of activation of catalyst

\item Post activation 3D study of extrudate

\item 2D + temporal measurement of operation of catalyst under H2 step

\item Post operation 3D study of extrudate

\end{enumerate}

Over 250,000 data sets have been collected equating to about 2.5Tb of data. The sheer number of
datasets requires a new approach to processing requiring reading and fast squeezing of edf CCD
image data. These features have now been incorporated into the latest version of EasyDD. Now the
data need to be processed.

* prepared from [Ni(en)(H20)4]Clb (en = ethylenediamine) precursor complex.

%\chapter[Performance Analysis and Bundled Software]{Performance Analysis and Bundled Software for a New Pixelated Energy-Discriminating Detector} \label{Performance}
%
%As part of the \HEXITECs\ project, performance analysis is now required on the latest 20x20
%pixelated energy- discriminating detector. Response from characteristic X-ray fluorescence lines
%(derived from metal foils) has been measured from each pixel on the device. The analysis involves
%comparing the 400 spectra derived from each foil experiment to investigate the behaviour of the
%device: looking at energy calibration, peak tailing, intensity response and additional formed
%features such as escape peaks. The \ProgName\ software is ultimately to be bundled with the
%finished detector system providing a tool to read and analyse recorded spectra. Several reading
%formats have already been incorporated into \ProgName. The performance analysis, outlined above,
%requires asymmetric peak fitting and development of statistical analysis tools. Some/all of these
%features need to be incorporated into the \ProgName\ software.
%
%To be moved to EasyDD chapter
%
%possible inclusion of nickel data processing as an example of speed and efficiency.


%%SSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSS
%\section{\ProgName\ Future Development} \label{EasyDDFutureDevelopment}
%%
%Future development for \ProgName\ may include:
%
%\begin{itemize}
%
%\item Implementing \whpade.
%
%\item Mapping data on a 3D grid (tab for each slice) according to the real space coordinates.
%
%\item Investigating other optimisation techniques such as \maxlik.
%
%\item Incorporating more scientific functionality such as corrections, deconvolution and final analysis.
%
%\item Investigating correlation of neighbouring \voxel s.
%
%\end{itemize}

%%SSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSS
%\section{Recommendations for Future Experimental Work}
%%
%Our recommendations for the future work are
%
%\begin{itemize}
%
%\item Extending the current
%
%\item Implementing other
%
%\item Implementing
%
%\end{itemize}
%
%%SSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSS
%\section{\ProgName\ Future Development} \label{EasyDDFutureDevelopment}
%%
%Future development for \ProgName\ may include:
%
%\begin{itemize}
%
%\item Implementing \whpade.
%
%\item Mapping data on a 3D grid (tab for each slice) according to the real space coordinates.
%
%\item Investigating other optimisation techniques such as \maxlik.
%
%\item Incorporating more scientific functionality such as corrections, deconvolution and final analysis.
%
%\item Investigating correlation of neighbouring \voxel s.
%
%\end{itemize}

possible table to include 2theta, d values and hkl for all identified peaks (59) sectioned
according to phase


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Nickel nitrate calcination
%\begin{enumerate}
%
%\item
%This PDP is observed at \sad\ = 1.03469, 1.24181, 1.37864, 1.79219, 2.0681, 2.18187, 2.30912,
%2.49171, 2.82742, 3.06858, 3.44747, 3.80158, 4.73755, 4.95967, 5.21861. It belongs to the nickel
%ethylenediamine dinitrate (\Nieddn) precursor. This is concluded from a comparison with the
%\Nieddn\ diffraction pattern obtained from Krishnan \etal\ \cite{KrishnanJS2009} after scaling the
%\scaang\ to match the wavelength.
%
%\item
%This PDP is observed at \sad\ = 2.92384.
%
%\item
%This PDP is observed at \sad\ = 5.37095.
%
%\item
%This PDP is observed at \sad\ = 6.56718, 8.53682, 8.6387.
%
%\item
%This PDP is observed at \sad\ = 6.33744.
%
%\item
%This PDP, which belongs to alumina, is observed at \sad\ = 4.02862, 5.70997.
%
%\item
%This PDP is observed at sad\ = 8.00588. It possibly belongs to other form of alumina.
%
%\item
%This PDP is observed at \sad\ = 0.411373, 0.554836, 0.451794. low scattering angle. possible
%pre-crystallization. check 0.554836 final position.
%
%\item
%This PDP is observed at \sad\ = 3.2909, 3.2926, 3.27499.
%
%\item
%This PDP is observed at \sad\ = 3.80212.
%
%\item
%This PDP is observed at \sad\ = 2.75323, 4.3953, 4.52958.
%
%\item
%This PDP is observed at \sad\ = 3.49647 3.48947 5.22459, 6.99423, 7.70071, 8.9887, 9.01788,
%9.88169.
%
%\item
%This PDP is observed at \sad\ = 6.33739, 7.61602.
%
%\end{enumerate}

%A sample of these peaks are presented as tomographic images in Figures (\ref{5p70997-Par3V8},
%\ref{2p30912-Par3V8}).
%
%\begin{figure} [!h]
%\centering
%\includegraphics
%[scale=0.65] {g/5p70997-Par3V8}
%%
%\caption{Tomographic images of the Gauss area of the nickel nitrate calcination data sets for the
%largest $\gamma$-alumina peak at $2\theta \simeq 5.75^{\circ}$.} \label{5p70997-Par3V8}
%\end{figure}
%%
%\begin{figure} [!h]
%\centering
%\includegraphics
%[scale=0.65] {g/2p30912-Par3V8}
%%
%\caption{Tomographic images of the Gauss area of the nickel nitrate calcination data sets for the
%largest \Nieddn\ peak at $2\theta \simeq 2.37^{\circ}$.} \label{2p30912-Par3V8}
%\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Nickel nitrate reduction
%\begin{enumerate}
%
%\item
%This PDP, which belongs to the alumina phase, is observed at \sad\ = 4.02862, 5.70997, 9.88169.
%Decay in intensity is observed for the $2\SA=$ 9.88169 peak. This PDP is also observed at $2\SA=$
%0.411373, 0.554836, 0.451794 but with increasing intensity at the beginning. This is a truncated
%peak (check).
%
%\item
%This egg yolk distribution is observed at \sad\ = 3.49647, 3.48947, 5.22459, 6.99423, 8.00588,
%9.01788.
%
%\item
%This circular pattern is observed at \sad\ = 1.57345, 1.79219, 2.0681, 4.67714; and it apparently
%belongs to a glass container used to keep nitrogen flow during reduction.
%
%\item
%This egg shell distribution is observed at \sad\ = 3.80212, 5.37095; and it belongs to (?).
%
%\item
%This PDP is observed at \sad\ = 3.2909, 3.2926, 3.27499, 6.33739, 6.33744. It apparently a mix of
%two phases, i.e. either 1 and 4 or 2 and 4.
%
%\item
%This PDP is observed at \sad\ = 6.56718, 8.6387, 8.53682. It is a mix of 3 and 5.
%
%\item
%This PDP is observed at \sad\ = 2.92384, 7.61602, 7.70071, 8.9887.
%
%\end{enumerate}


%A sample of tomographic images of the reduction data sets are presented in Figures
%(\ref{4p02862-Par3V17}, \ref{3p80212-Par3V17}, \ref{6p33744-Par3V17}).
%
%\begin{figure} [!h]
%\centering
%\includegraphics
%[scale=0.65] {g/4p02862-Par3V17}
%%
%\caption{Tomographic images of the Gauss area of the nickel nitrate reduction data sets for the
%second largest $\gamma$-alumina peak at $2\theta \simeq 4.08^{\circ}$.} \label{4p02862-Par3V17}
%\end{figure}
%%
%\begin{figure} [!h]
%\centering
%\includegraphics
%[scale=0.65] {g/3p80212-Par3V17}
%%
%\caption{Tomographic images of the Gauss area of the nickel nitrate reduction data sets for a peak
%at $2\theta \simeq 3.8^{\circ}$ most likely belongs to \Nieddn.} \label{3p80212-Par3V17}
%\end{figure}
%%
%\begin{figure} [!h]
%\centering
%\includegraphics
%[scale=0.65] {g/6p33744-Par3V17}
%%
%\caption{Tomographic images of the Gauss area of the nickel nitrate reduction data sets for a peak
%at $2\theta \simeq 6.3^{\circ}$ most likely belongs to \Nieddn.} \label{6p33744-Par3V17}
%\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Nickel chloride
%\begin{enumerate}
%
%\item
%This PDP is observed at \sad\ = 0.850868, 1.58641, 1.65566, 1.80608, 2.49495, 2.67527, 2.77194,
%3.89095, 4.75318, 4.76549.
%
%\item
%This PDP is observed at \sad\ = 1.11398, 1.58634, 1.65588.
%
%\item
%This PDP is observed at \sad\ = 0.935951, 1.48064, 2.29245, 2.89994, 3.02421, 3.1669, 3.02342,
%3.16562. The shadow in Figure \ref{NiCl2ndMask1}at frames 4-7 are coming from the neighbouring peak
%at about \sad\ = 0.85 (check), as seen in Figure \ref{NiCl2ndStackBP1}.
%
%\item
%This PDP is observed at \sad\ = 3.76146, 5.17819, 6.16946, 6.67435, 7.22707, 7.37335.
%
%\item
%This PDP is observed at \sad\ = 1.40004, 4.88798.
%
%\item
%This PDP is observed at \sad\ = 2.96369, 2.97309, 3.25362, 3.25587, 3.49617, 3.69953, 4.9436,
%5.06598.
%
%\item
%This PDP is observed at \sad\ = 4.39349.
%
%\item
%This PDP is observed at \sad\ = 3.99338, 4.00304, 4.61186, 6.5262, 7.65856, 7.99623, 10.3352,
%11.3301, 12.0233. the shadow ring comes from the neighbouring peak at \sad\ = (check).
%
%\end{enumerate}

This is concluded from a comparison with the \Nieddn\ diffraction pattern obtained from Krishnan
\etal\ \cite{KrishnanJS2009} after scaling the \scaang\ to match the wavelength.

%Most crystallographic phases of this collection are already identified by Simon Jacques (SJ). In
%this section we present the details that we worked out guided by the SJ identification.


More than 60 confirmed and suspected peaks were identified from the stack plots and curve-fitted to
the actual diffraction patterns of the individual pixels.

The 0.45 degree feature should belong to alumina or ethylenediamine because it exists in both
nickel nitrate and nickel chloride data. It is also seen truncated in molybdenum data. Note that
the unidentified phase (1-0p466915-Par3\_1) increases while alumina decreases, as if alumina is
transforming to this phase.

Mo sixth: 1.41, 1.88, 1.99, 2.19, 2.36, 2.51, 2.82, 3.10, 3.71, 4.33, 4.97, 5.22, 6.01, 6.33,

Mo seventh: 2.10, 2.36, 2.75, 3.40, 4.37, 4.84, 5.03, 5.53, 6.44?

%However, one exception is that of Repelin and Husson \cite{RepelinH1990} which gives two peaks at
%\sad\ = 0.35 and 0.69; it might be that the above phase peak at \sad\ = 0.42 derives from these two
%overlapping peaks.

%\item
%The sixth and seventh PDPs apparently belong to molybdenum dioxide MoO$_2$. The
%sixth is observed at about \sad\ = 1.41, 1.88, 1.99, 2.19, 2.36, 2.51, 2.82, 3.10, 3.71, 4.33,
%4.97, 5.22, 6.01 and 6.33; while the seventh is observed at about \sad\ = 2.10, 2.36, 2.75, 3.40,
%4.37, 4.84, 5.03, 5.53. The following peaks of MoO$_2$-[P42/MNM] \cite{SeisenbaevaSNDK2004} may
%have link to the previous peaks: (\sad, $hkl$, $d$ \AA) = (2.36, 110, 3.4276), (3.34, 200, 2.4237),
%(3.72, 111, 2.1747), (4.72, 220, 1.7138), (5.28, 310, 1.5329), (5.53, 221, 1.4636) and (6.01, 311,
%1.3461). Other peaks that may belong to this phase and could be masked due to closeness of other
%peaks include: \sad\ = 3.32, 5.75, 5.77 and 7.81.
%%Also the peaks at the following scattering angles have a shadowy trace on the tomographic image or
%%the stack plot: \sad\ = 6.65, 7.08 and 7.46. These peaks are suspected to be from this phase.


%EasyDD the objective of creating a software designed for the treatment of large volume of
%diffraction data; specifically for treating:
%
%\begin{enumerate}
%
%\item Existing and future data derived from the three-angle \diffractometer s currently operating in
%a number of stations of \synrad\ facilities.
%
%\item New data derived from the multi-pixel energy dispersive detectors and collimators currently under
%development, such as multi-\TEDDIs\ detector under development by \HEXITECl\ (\HEXITECs) project.
%
%\end{enumerate}

%%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
%\section{Statement of intent}
%
%The principal objective of \ProgName\ project is to develop a computer code for batch fitting and
%bulk analysis of large volumes of diffraction data sets, mainly those obtained from synchrotron
%radiation sources. Such a utility greatly assists studies on various materials systems and enables
%far larger detailed data sets to be rapidly interrogated and refined. The recent development in
%multidimensional detectors such as those developed by \HEXITECs\ project highlights the need for
%such programs so that the data production power will be matched with data processing power.
%
%We are not aware of the existence of an all-encompassing software for diffraction imaging. For
%example, currently there are no tools to easily handle data derived from such experiments. Although
%the creation of such a software as part of a PhD program may be too ambitious, it is a necessary
%first step which can be built on in the future by the author or by other researchers. The demand
%for such a utility is becoming more obvious in the recent years with the improvements in
%instrumentation associated with increasing availability of bright \Xray\ source (e.g. third
%generation \synch s) and fast multi-dimensional detectors.
%
%In this PhD project we are aiming to develop the imaging techniques for the specific purposes of
%observing industrial \hetcat s in preparation and under action. Our intention is to build a
%software package that contains the tools to analyse the volume of data you expect from imaging
%studies.

The other peaks are either faint or masked by neighbouring peaks from other phases or are
duplicates due to splitting.


Peak splitting was observed in both ADD and EDD data but it was more prominent in the ADD data. The
splitting may be explained by sample size, lozenge size and shape, actual incident and diffracted
beam path (length and nature of material in the path) which causes absorption, distortion and
exciting other types of signal such as fluorescence.




%


==> Store.tex <==
%

Pecharsky and Zavalij\cite{BookPecharskyZ2005}: Smoothing is a numerical conditioning procedure
employed to suppress statistical noise, which is present in any powder diffraction pattern as a
result of random intensity measurement errors (Eq. 3.8 in Chapter 3). It improves the appearance of
the powder diffraction pattern. For example, smoothing can make quickly collected data (say in a 15
min experiment) look similar to a pattern collected in a longer (e.g. in an overnight) experiment,
and may help with certain automatic procedures, such as background subtraction, Ka2 stripping and
unbiased peak search. Numerical conditioning, however, does not improve data quality. Moreover, it
causes broadening of Bragg peaks and loss of resolution (e.g. see Figure 3.38 and Figure 3.39 in
Chapter 3, which illustrate broadening caused by the varying receiving slit) and may result in the
disappearance of weak peaks when overdone. On the contrary, increasing experiment time improves the
pattern since it reduces statistical spreads. An example of the original and smoothed patterns is
shown in Figure 4.5.

Book Will 2006: Powder diffraction is based on a statistical distribution of many crystallites. To
determine the true relative intensities a completely random orientation of the crystallites is
required by theory. Specimen with completely random orientation however are hard, if not impossible
to prepare. Therefore corrections are necessary. After taking precautions and care in the
preparation of the specimen and in the experiments a mathematical correction is necessary in the
course of the refinement and such corrections are provided in all refinement programs in use.

Book Will 2006: Powder diffraction is based on a statistical distribution of many crystallites. To
determine the true relative intensities a completely random orientation of the crystallites is
required. Such specimens however are hard, if not impossible to prepare. Therefore precautions are
necessary in the experiments and corrections through calculations must be made in the evaluation.

David 2004: The Rietveld method is the most straightforward and statistically correct approach for
the re®nement of crystal structure parameters from powder diffraction data. The equivalent
two-stage approach, involving the re®nement of structural parameters based on integrated
intensities extracted using the Pawley method, is extremely useful in circumstances such as the
global optimization methods of structure determination, where a great many re®nements need to be
performed very quickly. The equivalence is emphasized in a simple mathematical relationship between
the goodness of ®ts obtained in Rietveld, Pawley and correlated integrated intensities re®nements.
A rationale is given for determining the estimated standard deviations for structural variables
from powder diffraction data.

David 2004: The advent and development of the Rietveld (1967, 1969) method has revolutionized
powder diffraction. Moderately complex structures may be re®ned with ease from powder diffraction
patterns using the Rietveld method in a stable manner since the approach correctly accounts for
Bragg peak overlap. Another approach, involving a two-stage process, was originally proposed by
Sakata & Cooper (1979). Their principal concern with the Rietveld method was that the simultaneous
re®nement of structural parameters and pro®le parameters, such as peak widths and cell constants,
would lead to biased estimates of the structural parameters. Prince (1985, 1993), in a detailed
exposition, presented an algebraic proof that the structure parameters obtained from the two
approaches were indeed the same. This fact is intuitively obvious since structural parameters are
obtained from the magnitudes of the integrated intensities, which are implicitly calculated with
due account of overlap in the Rietveld method. There are three important consequences of this
equivalence. Firstly, careful use of the Rietveld method with the correct pro®le and structural
models offers the most straightforward unbiased approach to structure re®nement from powder
diffraction data. Secondly, the `two-stage' integrated intensity method also provides the correct
answer, although neglect or incorrect evaluation of the correlations in the `two-stage' method
leads necessarily to incorrect estimated standard deviations and, if the structural model has
substantial de®ciencies, also to incorrect structural parameters. Note that, although the term
Pawley analysis is used to describe the least-squares re®nement of integrated intensities, the
original Pawley (1981) program does not generally provide the correct correlated intensities. In
particular, the introduction of slack constraints, as additional observations (Waser, 1963), to
avoid negative intensities, although elegant, results in unwanted bias. The third important
consequence of equivalence is associated with speed of calculation. While use of the statistically
correct `twostage' method is an unnecessary complication for a standard Rietveld re®nement, the
initial extra effort introduces a substantial timesaving at the stage of evaluating the ®t of the
model to the data. A particularly pertinent example is in the area of structure determination using
global optimization strategies, where very large numbers of powder diffraction patterns calculated
from trial structures must be compared with an observed powder diffraction pattern. The present
paper illustrates clearly the relationship between the Rietveld and two-stage methods in
mathematical and practical terms. Particular attention is drawn to dealing with background
estimation and estimation of errors in the re®ned model.

Dong S 1999: The modelling of powder diffraction patterns is of considerable interest in several
fields of study, from crystallography to materials science. Besides the obvious application to
separate the contribution of Bragg re¯ections in the case of peak overlap, profile fitting is the
basis of the Rietveld method (Rietveld, 1969; Young, 1993) and is increasingly used for
line-profile analysis (LPA) and lattice-parameter determination (Langford, 1992; Langford & LoueÈ
r, 1996; Toraya, 1993). The latter two applications do not require any treatment of the information
related to peak intensity and area, which can be considered as fitting parameters to be optimized
during the modelling of the pattern. The interest in this approach lies in the modelling of peak
positions, with possible inclusion of an internal standard, and profile parameters (width and
shape). This type of analysis is referred to as the Pawley method (Pawley, 1981; Snyder, 1993;
Toraya, 1993) or, more generally, whole-powder-pattern fitting (Scardi, 1999). Besides the obvious
interest in the study of lattice parameters, diffraction domain size and lattice defects, an
advantage of this procedure is that it does not require a structural model of the phases present;
moreover, the material to be studied need not be pure, as additional diffraction peaks can be
easily included to model peaks from impurities or unknown phases.

Dong S 1999: The base algorithm was conceived to work as an unconstrained profile fitting (Pattern
decomposition) or a constrained modelling of the whole powder pattern (Pawley method), by which
peak positions or lattice parameters, respectively, can be refined by least squares.

Getting Started with Rietveld -Rv -p: probability of finding an incorrect structure model that is
both plausible and is in good agreement with the diffraction observations is very small (but not
zero!). Computer-assisted least-squares optimization allows structural models to be improved,
limited only by the quality of the data

Getting Started with Rietveld -Rv -p: Hugo Rietveld realized that if a pattern could be modeled,
the fit between these data and the a computed pattern could be optimized.

reread "Getting Started with Rietveld -Rv -p"

Getting Started with Rietveld -Rv -p: Disadvantage of Rietveld: Many parameters need to be fit Ä
Background – fixed – functions Ä Peak shape – "fundamental parameters" – functions Ä Lattice
constants – zero correction – flat plate terms Ä Scaling – Phase fractions Ä Structural parameters
– atom positions – occupancies – displacement parameters Ä Preferential Orientation Ä Absorption

Gilmore 1996: Bayes's theorem, on which Bayesian statistics is based, appears in many guises. It
was first derived by the 18th century English clergyman and talented mathematician Thomas Bayes,
and found in his papers on his death. [See Molina (1963) for a reprint of this paper and a critical
discussion.] It was rediscovered by Laplace, who used it to solve a wide variety of outstanding
problems in astronomy. At its simplest, the theorem is uncontroversial. Let us suppose that we are
carrying out an experiment to gain information on a parameter 0. Before commencing the experiment,
we have prior belief of the possible values of 0, which we express as an unconditional probability
distribution p(O). If the experiment yields data represented by the vector x, then Bayes's theorem
states p(01x) (x p(xlO)p(O). (12) The constant of proportionality may be determined by
normalization. The term p(01x) is called the posterior distribution (or simply posterior); the
function p(xl0) is the likelihood, which consults the data from the experiment, and p(O) is the
prior probability. As written, this is an uncontroversial equation simply derived from the axioms
of probability theory and used by all statisticians to invert conditional probabilities, i.e. to
obtain p(xl0) from p(01x) and vice versa. However, Bayesian statisticians take the topic a whole
step further by using (12) as a model of scientific inference. In addition, probabilities are
defined not in the narrow frequentist way but in the broader, and much more controversial, sense of
degree of belief, which is ideally suited to science where measurements can be very difficult to
relate to frequencies without the use of very convoluted argument, and a counter-intuitive use of
language. Furthermore, (12) is used iteratively: the posterior becomes an updated prior and the
whole cyclic process repeated until convergence is reached. From these departures from classical
statistical methods stem a great deal of sometimes very acrimonious dissent. (See, for example,
Jaynes 1979.)

Gilmore 1996: A common objection to the use of Bayes's theorem is that a systematic error or bias
in the prior p(O) will give rise to similar errors in the posterior p(01x). The use of the
likelihood, i.e. the intervention of the experimental data, makes this less of a problem than may
appear at first but the ME formalism becomes a very powerful tool here: we chose a prior via
maximum entropy, which has a minimum bias and is maximally non-committal towards missing data. This
is then an optimal prior for use with Bayes's theorem.

possible use of "Gilmore 1996" paper for statistics in crystallography

Gilmore BB 1989: It is clear that the maximumentropy method is a powerful tool for phase
determination and, when combined with likelihood, is capable of solving the crystal structures of
small organic molecules. Likelihood is a unique discriminator of phase sets when used as a figure
of merit in a multisolution environment, and also an equally powerful tool in phase refinement.

"Gilmore BB 1989" is an example of using statistical techniques and approach

Gilmore papers in general as example for statistical methods

Gilmore HB 1991: Traditionally, structures are difficult to solve ab initio from powder diffraction
data because of peak overlaps, which arise accidentally or are imposed by point-group symmetry.
Overlaps reduce both the effective sampling of reciprocal space and the resolution of the data;
this makes the application of traditional direct methods difficult. In the method of combined
entropy maximization and likelihood evaluation described here, the intensity data are normalized
using both the overlapped and non-overlapped reflections by means of a suitably modified version of
the MITHRIL computer program

Gilmore HB 1991: We have demonstrated the applicability of the combined use of entropy maximization
and likelihood estimation to the determination of crystal structures from their X-ray powder
diffraction patterds even when the data are relatively poor in quality. The single-crystal
likelihood, calculated from non-overlapped reflections, is a poor discriminator in these
circumstances, but the new likelihood incorporating the overlap information has proved to be a
uniquely powerful figure of merit. Entropy serves as a valuable secondary indicator of preferred
phase sets.

Glazer HB 1978 -p: In recent years there has been an upsurge of interest in powder diffraction,
particularly since the work of Rietveld (1969). This work showed that it was possible to 'lift out'
the intensity contributions of the component overlapping reflections inherent in powder diffraction
by performing least-squares refinement of the usual structural parameters, and by taking advantage
of the known Gaussian line-shape of neutron diffraction peaks. The process also includes in the
least-squares refinement parameters relating to the half-widths of the Gaussian peaks, peak
asymmetry and preferred orientation, the counter-zero position and the lattice parameters. The
result is that structural refinement can be carried out very rapidly with good precision for the
coordinates, although the reliability of the temperature factors obtained is still a matter of
concern.

Honkimaki S 1992: An unambiguous separation of the Bragg reflections from the total observed powder
diffraction pattern requires a correct model for the profile of the reflections and the background.
The profile is due to instrument factors and sample effects or external and internal factors. For a
well characterized instrument, the profile function due to the external factors can be calculated
by ray tracing. The internal factors include the effects of crystalline size, faulting and strains,
and typically they are modeled by Gaussians and Lorentzians, which have angle-dependent widths. In
this way the number of non-structural parameters of the model is minimized and the remaining ones
characterize the sample (Suortti, 1991). Almost all treatments of backg'ound assume a slowly
varying function, which is fitted to the observed pattern at points where Bragg reflections do not
contribute. This criterion is more or less subjective and based on conventions which may not be
justified. The form of the background is obviously related to the profile function used for the
Bragg reflections and particularly the thermal-motion parameters are strongly affected by this
choice (Ahtee, Unonius, Nurmela & Suortti, 1984). There are some schemes where the Bragg
reflections and the background are fitted simultaneously, using analytical functions (Wiles &
Young, 1981). In a more fundamental approach, the components of background are described by
functions that have the correct average behavior (Sabine & Clarke, 1977). The aim of this work is
to go one step further by deriving a general presentation for the diffraction pattern where all
components of scattering have correct angular dependencies and where all the parameters are related
to the crystal structure or to the sample properties.

Honkimaki S 1992: The Rietveld refinement is based on fitting the structural model directly to the
total pattern of Bragg reflection profiles. This was unnecessary in the present case where the
profiles were calculated precisely from diffraction geometry. However, the present ideas can be
adapted to the Rietveld method quite easily even when the profile shapes are determined by the
sample factors. The profile shapes are described with a sufficiently versatile function, such as
the Voigtian, and the angular dependencies are given by two functions that model the effects of
crystalline size and microstrains. The parameters of the functions are refined in fitting the
model. These intrinsic profiles are convoluted by the instrument function, which is calculated from
the geometry of the experiment as in the present work. The structure factors and Debye- Waller
factors of the model are used to calculate the TDS intensity. In this way, all the parameters of
the model are related to the sample properties, not to those of the instrument.

Jansen SW 1988: For accurate structure analysis, i.e. the precise determination of the integrated
intensities, the background and its variation with angle must be known and have to be determined.
Principal sources of background are insufficient shielding, electronic noise of the detector system
and the sample itself due to diffuse and incoherent thermal neutron scattering, TDS and others
(Sabine, 1980). There is no well established theoretical approach to the background. Background,
therefore, may be determined by analytical procedure or by a polygon fit through manually selected
footing marks in the powder pattern (Rietveld, 1969).

Joubert 2002: While being the most efficient way of analyzing a powder diffraction diagram for
evidencing an additional phase, refining lattice parameters and performing quantitative phase
analysis, the Rietveld method is also able to perform structure refinement including accurate
determination of atomic positions and atom occupancies at the different sites. Owing to
technological improvements of both powder diffractometers, and Rietveld analysis software, the
method is now able to compete with single crystal analysis. It is actually the only alternative
when single crystals do not exist or when no single crystal diffractometer is available. The
Rietveld method makes possible the determination of vacancy ratio or relative occupancies when
atoms of different kinds can occupy the same sites. It allows the measurement of the order
parameter in partially ordered structures and the determination of the mechanism for accommodating
the excess or deficient atoms in non-stoichiometric phases. This makes the Rietveld method the
ideal tool to use in conjunction with the sublattice model especially if experimental site
fractions can be taken into account in phase diagram assessment software. Powder diffraction
associated with Rietveld analysis should therefore be widely used as an efficient experimental tool
for thermodynamic optimization.

Joubert 2002: The Rietveld method is a structural refinement method not to be confused with a
structural determination method. That means that the crystal structure type of the phase studied
has to be known prior to the analysis as well as approximate lattice parameters before attempting
any refinement.

Joubert 2002: A pattern is first calculated from the known structure information: the nature of the
phases in the sample, atomic positions and the nature of the atoms at each site according to the
structure prototype, approximate line profiles and lattice parameters. The calculated pattern is
compared with the experimental (observed) one and the parameters defining the calculated pattern
are iteratively refined by a non-linear least-square method in order to obtain the best agreement
between the two patterns, by minimizing the function: where y stands for the observed (ohs) and
calculated (talc) intensities, the summation being done over each point of the diffraction pattern.
The parameters, which can be refined and therefore experimentally determined include background
parameters, line profile parameters (derived from the observed line shapes), lattice parameters
(derived from the observed line positions), atomic positions, displacement factors and occupancy
factors (derived from the line intensities). This paper will be devoted to what can be obtained
from this latter parameter in the frame of the thermodynamic modeling of a particular phase.

Langford L 1996 -p: New approaches for the treatment of powder data have been devised, based on
maximum entropy methods and 'simulated annealing', for example, to generate structural models.

Louer M 2000: Powerful methods are available for pattern indexing, extraction of integrated
intensities, structure solution and refinement of the structure model with the Rietveld method.
Efficient Rietveld programs are available, among them the most popular are FULLPROF from
Rodriguez-Carvajal (F), GSAS from Von Dreele (USA) and RIETAN from Izumi (J).

Louer M 2000: Most important methodological advances in powder diffraction, even until today, are
due to European contributions (see section 2.2). On the other hand, (dedicated) applications are
most advanced in the USA and Japan. It is striking to note that the International Centre of
Diffraction Data (ICDD) is an USA organisation. Only relatively recently in Europe the European
Committee for Standardisation (CEN/TC 138) started an extensive project on the use of diffraction
methods.

McCusker DCLS 1999: Background contribution There are basically two approaches to dealing with the
background in a powder diffraction pattern. It can either be estimated by linear interpolation
between selected points between peaks and then subtracted, or it can be modelled by an empirical or
semiempirical function containing several re®nable parameters. Both have their advantages and
disadvantages. For a simple pattern where most peaks are resolved to the baseline, both methods
tend to work well and the ®t is easily veri®ed with a plot. For complex patterns with a high degree
of re¯ection overlap, however, the majority of the peaks are not resolved to the baseline, so the
estimation of the background is dif®cult. This means that if a backgroundsubtraction approach is
used, the background usually has to be re-estimated and re-subtracted several times during a
re®nement. The background variance is also dif®cult to estimate and is often assumed to be zero.
However, it should be taken into account if the weighting scheme used in the re®nement [usually
1/[2(I)] is to be correct. While background subtraction can be a somewhat cumbersome approach to
background correction and may seem to be rather unsophisticated, it has the advantage of being
¯exible. It might appear that re®ning the background would be the preferred method, because this
would eliminate some of the problems inherent to background subtraction (i.e. the background and
structural parameters can be re®ned simultaneously and the standard deviations estimated in the
usual way). However, the polynomial functions usually used for this purpose are largely or entirely
empirical. If the polynomial happens to describe the background well, then, as might be expected,
this procedure also works well; but if it does not, no amount of re®ning the coef®cients of the
polynomial (or increasing the order of the polynomial) can correct the problem and the re®nement
will not proceed satisfactorily. In such a case, background subtraction is the better approach. Of
course, it is also possible to use the two techniques in combination. A simple empirical function
can be used to ®t the background and then the deviations described by a sequence of ®xed points.
The advantage is that the magnitude of the ®xed part is minimized and thus the impact of its
inherent arbitrariness on the re®nement is reduced.

Riello FC 1998: the scale factor that transforms powder intensities from arbitrary units into
electron units is proposed.

Rietveld 1988: With the arrival of the larger Electrologica X8 computer, the program was written in
its recent form and includes the capability of refining structure as well as profile parameters

Rietveld Method presentation: this is important. read it again!


%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
\section{Constraints and Restraints} \label{ConstraintsRestraints}

Constraint: A rigorously applied limit

Restraint: A loosely applied limit

Restraints or soft constraints are relations between parameters of the model that are treated
formally in the same way as observations (Waser, 1963; Hendrickson \& Konnert, 1980; Hendrickson,
1985). They may be used to specify bond lengths, angles, planarity of molecules, relations between
displacement parameters, and for numerous other purposes. The uncertainties attributed to such
pseudo-observations are chosen according to the scientist's beliefs regarding their validity, in
agreement with the Bayesian interpretation of statistics. S.u.s of the parameter estimates are, of
course, dependent on these variances. It may be difficult to judge whether they are appropriate if
they are recorded in a structure data file omitting all information regarding the restraints.
(Schwarzenbach \etal\cite{SchwarzenbachAFGHe1989})

Pecharsky and Zavalij\cite{BookPecharskyZ2005}: A constraint is an exact mathematical relationship
existing between two or more parameters; it completely eliminates one or more variables from the
least-squares refinement. For example, y = x, and B33 = BZ2 = BI1, eliminate y, and B33 and B22,
respectively (also see Eq. 7.9). A restraint is additional information, which is subject to a
probability distribution. For example chemically (but not symmetrically) identical bond lengths in
tetramethylarnmonium

Least Squares Refinement: Crystallographic least squares cannot sensibly be discussed without
reference to constraints and restraints, which are an inevitable feature of structure refinement.
Their proper use makes the difference between getting a significant physical solution, and just
getting numbers out of the program. The major advantage of constraints is that they reduce the size
of the computation. Restraints offer the advantage of great flexibility, and an indication of when
they are inappropriate. A 'reasonable' restraint which is strongly disobeyed (Yc very different
from Yo) after refinement is a good indication of either some serious problem with the data, or
that the restraint is inappropriate, in which case you have mis-understood the model.

Likelihood theory and application to structure refinement: As noted above, a big problem with
macromolecular structure determination is the poor observation:parameter ratio at the resolutions
to which crystals normally diffract. If we simply refine the positions and B-factors of all the
atoms, the refinement will be poorly behaved, the data will be terribly overfit, and the resulting
atomic model will probably be very poor. The way we deal with this is either to add "observations"
in the form of restraints, or reduce the number of parameters by constraining the model in some
way. Typical restraints include bond lengths, bond angles and van der Waals contact distances.
There are generally also restraints to keep planar groups planar, and to maintain the chirality of
chiral centres. The restraints are entered as terms in the refinement target, and are weighted so
that the deviations from ideal values match the deviations found in databases of high resolution
structures. Constraints are a bit different. When you constrain a structure, you are actually
changing the parameterisation to reduce the total number of parameters. One possibility is to allow
only torsion angles to be adjusted, instead of all the individual x,y,z coordinates. Another very
common case occurs when there are multiple copies of a molecule in the asymmetric unit of the
crystal. The model can be a single copy of the molecule, replicated by rotations and translations
to create the other copies. So if, for instance, there are three copies in the asymmetric unit, the
number of adjustable parameters can be reduced by a factor of three. It turns out that there is a
way of looking at likelihood that brings restraints in naturally, by interpreting the restraints as
bringing in the a priori probability of different possible models. To understand this requires us
to digress a bit into more likelihood theory.

Likelihood theory and application to structure refinement: Bayesian interpretation of restraints In
structure refinement, restraints to ideal geometry can be thought of as expressing the a priori
probability of the model. In this analysis, any prior information about the probability of certain
features in real proteins could legitimately be introduced. In any event, we need restraints to get
around the problems of the typical parameter to observation ratio in protein structure refinement,
which was mentioned above. Restraints supply information about the allowed geometry of the
molecules we are dealing with: bond lengths, bond angles, van der Waals contacts, even preferred
torsion angles. In terms of likelihood theory and the Bayesian interpretation, restraints should
have a basis in probabilities. For instance, a bond length could be given a Gaussian probability
distribution from small molecule observations. This will enter the log likelihood target as a
weighted squared deviation

%XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX

Louer M 2000: The advent of the Rietveld method by Rietveld (NL) in 1967, combined with indexing
procedures, has contributed to the renaissance of the powder method in opening the door to ab
initio structure determination. The initial applications in the 80s were essentially due to
European researchers, e.g. Werner (S), Cheetham (UK) and Louër (F). Application of synchrotron
X-rays occurred first in 1983 by Cox et al. (USA), and later in European centres. New approaches
have been developed for quantitative analysis by Hill and Howard (Australia) and for structure
analysis. For instance, algorithms for extracting integrated intensities have been proposed by
Pawley (UK) and Le Bail (F). Direct methods have been adapted to powder data by Giaccovazzo et al.
(I) and Rius (S), simulated annealing and genetic algorithm by David et al. (UK) and Harris et al.
(UK). Microstructure analysis has profited from the introduction of the Voigt function in 1978 by
Langford (UK) and the use of pattern fitting to extract microstructural parameters in the 80s by
Mittemeijer et al. (NL). The interpretation of dislocation densities in diffraction line profiles
has been first introduced by Krivoglaz (Ukraine).

the analysis was extended to profile fitting and pattern decomposition, which allowed one to
extract individual intensities from overlapping diffraction peaks. This moved powder diffraction
into the neighborhood and even in competition to single crystal structure analysis
(Will\cite{BookWill2006}).


Jansen SW 1988: A profile fitting routine performs a least-squares fit of a (given) profile
function to the diffraction pattern by minimizing the second norm of the residuals
%
\begin{equation}\label{funcMinimise}
    \funcMin = \sum_{i} \wei_{i} \left(  \yobs_{i} - \ycal_{i} \right)^{2}
\end{equation}
%
with the summation index $i$ over all points in the diffraction pattern. The range of the segment
to be fitted is adjustable by the user. Typically the number $n$ is of the order of 4000 to 15 000,
with, for example, 40 to 100 points per degree representing 40 to 150 degrees. The weights
$\wei_{i}$ are estimated and taken from the experimental error margins ai, which are assumed to be
proportional to the square root of the count rate yobs following Poisson counting statistics,
%
\begin{equation}\label{weiSigma}
    \wei_{i} = 1 / \VAR_{i}
\end{equation}


Will\cite{BookWill2006}: Profile fitting and pattern decomposition programs, especially using the
Two Stage method, allow one to extract individual intensities, thereby determining intensities
without knowledge of symmetry or structure of the compound. This opens the way to use powder
diffraction data for ab initio structure determination by conventional methods, like with Patterson
maps, through Fourier calculations or by "direct methods".

Lou\"{e}r\cite{Louer1998}: The most commonly used line-shape functions are derived from the
Gaussian (G) and the Lorentzian (L). The pseudo-Voigt function is the sum of G and L components, in
which is the mixing factor ( . 1 for L and 0 for G). The Pearson VII function is (L)m, where the
exponent m is the line-shape parameter (m . 1 for L and m.1 for G). The Voigt function is a
convolution of L and G components whose limits of application are defined by the value of the shape
parameter ', de®ned as the ratio of the full width at half the peak intensity (FWHM) to the
integral breadth (L), i.e. 0.6366 for L and 0.9394 for G. In practice, errors often arise from an
unavoidable truncation of line tails, particularly for line pro®les with Lorentzian trends (Toraya,
1985).

In this method (pattern decomposition), positions of Bragg peaks are established from lattice
parameters and symmetry. Only unit cell dimensions are refined and the resulting peak positions are
not `observed' but rather calculated from the refined lattice parameters. Peak shapes are dependent
on a few free variables in relevant analytical functions of Bragg angle, as was described in
Chapter 2, section 2.9. The integrated intensities, however, are determined individually for each
Bragg reflection. This method extracts quite reliable individual intensities and, hence, is a
typical data processing step that precedes the structure solution from first principles, as will be
discussed in Chapter 6. It is worth noting that the full pattern decomposition approach is used
increasingly often to obtain accurate lattice parameters when a powder pattern has been indexed but
the crystal structure remains unknown or is not of interest for a specific application. Preliminary
treatment of powder diffraction data and their conversion into reduced powder patterns for phase
identification and a database search are nearly always included as parts of data processing
software suites, which are available with the purchase of a powder diffractometer. Perhaps this is
the main reason explaining the lack of comparable freeware (Pecharsky and
Zavalij\cite{BookPecharskyZ2005}).


%%%%%%%%%%%%%%%%%%%%%%%
Ortiz CBGC 2000: It is well recognized that the use of the Rietveld method4,5 has many advantages:

Ortiz CBGC 2000: whereas traditional procedures make use of selected individual reflections in
order to estimate the weight fractions, in the Rietveld method all reflections for each phase are
included in the Rt, then minimizing the problem of overlapped peaks;

Ortiz CBGC 2000: in the techniques that use integrated intensities of individual peaks, the
presence of preferred orientation effects constitutes a serious drawback to obtain reliable results
in quantitative analysis. However, in the Rietveld method the texture effects can be considered in
the fitting process, leading to a more accurate estimation of relative phase proportions;

Ortiz CBGC 2000: in addition, the amount of information that we need for quantitative analysis in
the Rietveld method is small and is related to the crystal structure of the phases, precluding the
need for a standard.
%%%%%%%%%%%%%%%%%%%%%%%

The Rietveld method of refining powder diffraction patterns was originally developed for neutron
diffraction with fixed wavelength. Later on it was extended to the Time of Flight (ToF) neutron
diffraction and X-ray Angle Dispersive (AD) and Energy Dispersive (ED) diffraction methods.

The statistical weights given to each observation $\wei_{i}$ are estimated and taken from the
experimental error margins which are usually assumed to be proportional to the square root of the
count rate $\yobs_{i}$ following Poisson counting statistics
%
\begin{equation}\label{weiSigma}
    \wei_{i} = \frac{1}{\VAR_{i}} = \frac{1}{\yobs_{i}}
\end{equation}
%
where $\VAR$ is the variance. This weighting factor, which is used in several refinement programs,
reflects only the statistical errors of counting for the observed intensities, and makes no
allowance for errors in the calculated intensities $\ycal_{i}$. If there are inadequacies in the
structural model, or if the assumed peak shape differs from the true shape, then the calculated
intensities will be in error. Moreover, for points on the profile which are close together the
errors are likely to be in the same direction, and this correlation between residuals is greater
the closer together are the profile points (Will\cite{BookWill2006}, Albinati and
Willis\cite{AlbinatiW1982}).

The most popular method in the physical sciences, and about the only one used in crystallography,
is the method of least squares, which minimizes the weighted deviance dTWd where d is an n vector
of deviates. The positive-definite n x n weight matrix W may be written as a product W = BTB. The
matrix B is not in general uniquely defined and may be specified for example as an upper-triangular
matrix, or alternatively as a symmetric matrix. Equation (4) then becomes Dw = dTBTBd, where Bd is
the vector of weighted deviates. If correlation terms of W are assumed to be negligible, W becomes
a diagonal matrix, and the quantity commonly refined in least squares is obtained (Schwarzenbach
\etal\cite{SchwarzenbachAFGHe1989})

Antoniadis \etal\cite{AntoniadisBF1990}: The problem is thus to find a set of parameters explaining
as well as possible the data through the postulated model (1). This is usually done by means of a
weighted least-squares procedure. However, when studies are made for the validity of the results
(e.g. Hill \& Madsen, 1984) a number of problems appears such as unexpectedly large values of
goodness- of-fit statistics in some data sets, unrealistic estimates of standard deviations in the
parameters etc. This leads to the practical conclusion that improving the data statistics further
and further (larger counting times) may lead to 'worse' results, which, abruptly said, is
apparently in contradiction with classical statistical theory. The present work is devoted to a
complete discussion of existing statistical methods used for the analysis of powder or
single-crystal diffraction data (fitting of rocking curves) and concerns a class of statistical
regression models that allow the experimentalist to extract the best possible information from his
experiment. Estimation proceeds by defining a measure of discrepancy between the data and a
corresponding set of fitted values generated by the model. In what follows, the maximum-likelihood
principle is used to obtain estimates of the parameters in a regression model when the experimental
errors are assumed to follow a Poisson or a Poisson-like distribution.

Izumi 2000: The latest version of a Rietveld-analysis program RIETAN-2000 has a couple of advanced
features: partial profile relaxation and whole-pattern fitting based on a maximum-entropy method
(MEM). Partial profile relaxation means that primary profile parameters of (nearly) isolated
reflections can be individually refined independently of secondary profile parameters.

Izumi 2000: The latest version RIETAN-2000 for angledispersive diffraction has grown into a
versatile program supporting whole-pattern fitting under partial profile relaxation by the
Rietveld, Le Bail, and maximum-entropy methods; Le Bail refinement under partial profile relaxation
will be published elsewhere. In each of these patternfitting methods, three methods of nonlinear
least squares can be used: \GauNew, Fletcher's modified Marquardt, and Powell's direction set
methods [3, 4]. Powell's method has proved to be most effective for escaping from local minima in
the three kinds of pattern fitting.

Langford and Lou\"{e}r\cite{LangfordL1996}: Entropy maximization and likelihood estimation. In
contrast to the previous techniques, the maximum entropy (ME) method attempts to solve the overlap
and phase problems simultaneously. The theoretical basis of the maximum entropy method has been
presented by Bricogne (1984), who later described the adaptation of this approach to solving
crystal structures from powder diffraction data (Bricogne 1991). The multisolution method of phase
determination, combining entropy maximization and likelihood evaluation, was extended to structure
determination by Gilmore, Henderson and Bricogne (1991). In this method, overlapping data are
treated in a rational manner. The method consists of considering an unknown structure as being
composed of chemically identified atoms with unknown positions. The latter are initially considered
as random with a uniform distribution in the asymmetric unit cell and the technique consists of a
gradual removal of this randomness. The method has been applied successfully to the determination
of the structure of LiCF3SO3 (Tremayne et al 1992). Detailed procedures for solving small crystal
structures ab initio by means of ME and powder-diffraction data were reviewed recently by Sudo,
Hashizume and Carvalho (1995). As a test of the technique, the multi-solution method was applied to
the determination of the structure of a low pressure phase of magnesium boron nitride Mg3BN3.

Detailed procedures for solving small crystal structures ab initio by means of ME and
powder-diffraction data were reviewed recently by Sudo, Hashizume and Carvalho (1995). As a test of
the technique, the multi-solution method was applied to the determination of the structure of a low
pressure phase of magnesium boron nitride Mg3BN3 (Langford and Lou\"{e}r\cite{LangfordL1996}).

Antoniadis \etal\cite{AntoniadisBF1990}: While in the field of profile fitting X 2 is widely
accepted as a reasonable measure of goodness of fit, other statistics for describing the goodness
of fit, not commonly used in the statistical literature, are still very popular among
crystallographers. Thus, the statistical behavior of, for example, the conventional agreement
factors Rp and Rwp are (see e.g. Young, Prince \& Sparks, 1982) worth a closer look: [see equations
in the paper]

Messerschmidt\cite{BookMesserschmidt2007}: The Maximum Likelihood Method In Section 7.2.1, the
maximum likelihood method was briefly introduced as another possibility for the crystallographic
refinement of macromolecular structures. The basic assumption in least-squares minimization is that
the conditional distribution of each Fobs or Iobs when the model is known as Gaussian with the
expected value Fobs or Iobs and known uncertainties. In Eq. (7.3), the conditional probability
distribution was used for the observed structure factor Fobs. In an X-ray diffraction experiment,
we determine the amplitude Fobs of the structure factor only. Since likelihood is proportional to
the conditional probability distribution of experimental data when the model is known, the form of
this conditional probability is needed. The best way to do this would be to find the joint
probability distribution of all structure factors, but this task is not trivial and requires a
large amount of computer memory and time. Therefore, all existing refinement procedures assume that
the errors in different reflections are independent, and this simplification still delivers useful
results. With this assumption, the required joint probability distribution of all structure factor
amplitudes has the form ...

Antoniadis BF 1990: In profile-fitting methods, frequently one wishes to choose between two models
which differ essentially in the number of parameters used to describe the pattern. A model with
fewer restraints, that is with a greater number of parameters, can usually be made to fit the data
better than can a more restrained model (when the parameters in a model are a subset of these in
another model we say that the two models are nested); the crystallographer is thus often tempted to
add more and more parameters to obtain better fits. It is therefore important to obtain a
convenient method which allows one to decide whether the increase in the number of parameters leads
to a significant improvement in the agreement between the observed and calculated patterns. This
can be done by hypothesis-testing procedures or model-selection criteria.

Antoniadis BF 1990: Thus, the improvement brought by ML to the complicated case of structural fits
through the Rietveld method will be, in most cases, hidden behind the dominating effects of a
collection of, more or less, unavoidable systematic errors. However, even though the gain may not
seem immediate, firstly, ML is basically more correct and is no more time consuming, secondly, it
may handle dispersion and/or detector- response corrections in a natural way (Antoniadis &
Berruyer, 1990). On the contrary, when the interest is in profile fitting itself, the gain with ML
is obvious, especially for low counting rates and because of the set of diagnostic tests which may
be designed.

Antoniadis BF 1990: Our main conclusion is to permit a priori a model as general as possible, then
use the data, together with the likely background, to suggest possible modifications to the
hypothesized model. The best sort of mechanism of this type seems to be an accurate residual
analysis which considers the adequacy of the modified model for each individual bin. This could
solve many of the practical problems encountered when fitting long-counting-time or
large-sample-size data.























%
















%

